Hindsight Foresight Relabeling for Meta-Reinforcement Learning

Meta-reinforcement learning (meta-RL) algorithms allow for agents to learn new behaviors from small amounts of experience, mitigating the sample inefficiency problem in RL. However, while meta-RL agents can adapt quickly to new tasks at test time after experiencing only a few trajectories, the meta-training process is still sample-inefficient. Prior works have found that in the multi-task RL setting, relabeling past transitions and thus sharing experience among tasks can improve sample efficiency and asymptotic performance. We apply this idea to the meta-RL setting and devise a new relabeling method called Hindsight Foresight Relabeling (HFR). We construct a relabeling distribution using the combination of "hindsight", which is used to relabel trajectories using reward functions from the training task distribution, and "foresight", which takes the relabeled trajectories and computes the utility of each trajectory for each task. HFR is easy to implement and readily compatible with existing meta-RL algorithms. We find that HFR improves performance when compared to other relabeling methods on a variety of meta-RL tasks.

==> alteration.tex <==
The original meta-RL objective (without any data sharing) defined in Section~\cref{subsec:metaRL} is:
%
\begin{equation*}
\max_{\theta, \phi} \mathcal{L}_{\text{orig}}(\theta, \phi) = \mathbb{E}_{\psi \sim p\left(\psi\right), (s_t, a_t) \sim \pi'(\theta,\phi) }\left[\sum_{t=1}^{\infty}\gamma^{t - 1}r_{\psi}\left(s_t, a_t\right)\right]; \quad \pi'(\theta,\phi) = f_{\phi}\left(\pi_{\theta}, \tau_{\text{pre}}, r_\psi\right)
\end{equation*}
%
Here, a task is sampled from $p(\psi)$ and a trajectory generated for this task $\tau_{\text{pre}}$ is used in the adaptation procedure $f_\phi$. Let $\tau_\psi$ denote any trajectory collected for a given task $\psi$. Similarly, let $\psi_\tau$ denote the task that was being solved when a given trajectory $\tau$ was generated. Using the definition of the utility function (Eq.~\ref{eq:utility}), we can rewrite $\mathcal{L}_{\text{orig}}$ as:
%
\[
\mathcal{L}_{\text{orig}}(\theta, \phi) = \mathbb{E}_{\psi \sim p\left(\psi\right)} \mathbb{E}_{\tau \sim q^{\dagger}(\tau|\psi)} [U_{\psi}\left(\tau\right) + \mathcal{H}_{q^{\dagger}(\tau|\psi)}]; \quad q^{\dagger}(\tau|\psi) \triangleq \delta_{\tau,\tau_\psi}
\]
%
where $\delta_{\tau,\tau_\psi}$ is the Kronecker delta and the entropy term is added since it is equal to zero. Let there a dataset of trajectories collected from the various tasks in the meta-RL training set, and let these be represented by a distribution $\tilde{q}(\tau)$. The joint sampling of tasks and trajectories in the above equation can then be rearranged from $p(\psi)q^{\dagger}(\tau|\psi)$ to $\tilde{q}(\tau)q^{\dagger}(\psi|\tau)$, where $q^{\dagger}(\psi|\tau) \triangleq \delta_{\psi,\psi_\tau}$ is another Kronecker delta. Now, let $p(\tau|\psi)$ be the distribution defined in Section~\cref{subsec:relabel_distr_math}:
%
\[
        p(\tau|\psi) \triangleq \frac{1}{Z(\psi)} p_1(s_1) e^{U_\psi(\tau)} \prod^T_{t=1} \mathsf{p}(s_{t+1}| s_t,a_t)
\]
%
It is straightforward to show the following equivalence:
%
\[
   \mathcal{L}_{\text{orig}}(\theta, \phi) = \mathbb{E}_{\tau\sim \tilde{q}(\tau)} \mathbb{E}_{\psi \sim q^{\dagger}(\psi|\tau)}[U_{\psi}\left(\tau\right) + \mathcal{H}_{q^{\dagger}(\tau|\psi)}] = - \text{D}_{\text{KL}} \big[\tilde{q}(\tau)q^{\dagger}(\psi|\tau) \: ||\: p(\psi)p(\tau|\psi)\big]   
\]
%
In Section~\cref{subsec:relabel_distr_math}, we obtain the optimal relabeling distribution as:
%
\[
   q^*\left(\psi | \tau\right) \propto p\left(\psi\right)e^{U_{\psi}\left(\tau\right) - \log Z\left(\psi\right)}
\]
%
Therefore, the modified meta-RL objective we optimize in this paper is:
%
\[
 \max_{\theta, \phi} \mathcal{L}_{\text{mod}}(\theta, \phi) = \mathbb{E}_{\tau\sim \tilde{q}(\tau)} \mathbb{E}_{\psi \sim q^{*}(\psi|\tau)}[U_{\psi}\left(\tau\right) + \mathcal{H}_{q^{*}(\tau|\psi)}] = - \text{D}_{\text{KL}} \big[\tilde{q}(\tau)q^{*}(\psi|\tau) \: ||\: p(\psi)p(\tau|\psi)\big]   
\]
%
By using Lemma 2 from~\citet{eysenbach2020rewriting}, we have that:
%
\[
\mathcal{L}_{\text{mod}}(\theta, \phi) -   \mathcal{L}_{\text{orig}}(\theta, \phi) \ge \mathbb{E}_{\tau\sim \tilde{q}(\tau)} \big[\text{D}_{\text{KL}} [q^{\dagger}(\psi|\tau) \: ||\: q^{*}(\psi|\tau)]\big] = \mathbb{E}_{\tau\sim \tilde{q}(\tau)} \big[ -\log q^{*}(\psi_\tau) \big]
\]
%
This result shows that, for fixed meta-parameters ($\theta, \phi$), using the optimal relabeling distribution increases the value of the meta-RL objective. 

{\color{red} [Opinion:] Not clear why altering the meta-RL objective by increasing its value matters from a theoretical point of view. Ideally, it appears that we should care more about the {\em original} meta-RL objective since at test-time, we don't have data sharing.}

==> improvement_theorem.tex <==
\begin{theorem}
Our relabeling distribution improves the meta-RL objective over the tasks in the training distribution by at least the KL divergence between the relabeling distribution and the original distribution:
\begin{equation}
    D_{\text{KL}}\left(q\left(\tau, \psi\right) || p\left(\tau, \psi\right)\right) - D_{\text{KL}}\left(q_{\tau}\left(\tau, \psi\right) || p\left(\tau, \psi\right)\right) \geq
    \mathbb{E}_{q_{\tau}}\left[D_{\text{KL}}\left(q\left(\psi | \tau\right) || q_{\tau}\left(\psi | \tau\right)\right)\right]
\end{equation}
\end{theorem}
\begin{proof}
Apply Lemma 2 from~\citep{eysenbach2020rewriting}.
\end{proof}


==> max_relabeling.tex <==
% In Section~\ref{sec:relabeling}, we derived a relabeling distribution over tasks. For each trajectory, we are assigning high probability mass to tasks for which it has high utility. This raises the question: Why don't we just assign each trajectory to the task for which it achieves the highest utility (hard max), rather than sampling from a softmax distribution? We have already shown that our relabeling distribution improves the MaxEnt meta-RL objective. Analogously, we can show that relabeling each trajectory with the task for which it achieves the highest utility improves the meta-RL objective sans entropy term.

% \begin{theorem}\label{max_relabel_theorem}
% Relabeling a trajectory with the task for which it achieves the highest utility maximizes $\mathbb{E}_{p\left(\psi, \tau\right)}\left[U_{\psi}\left(\tau\right)\right]$.
% \end{theorem}
% \begin{proof}
% The meta-RL objective can be written as 
% \begin{equation*}
% \mathbb{E}_{p\left(\psi, \tau\right)}\left[U_{\psi}\left(\tau\right)\right] = \int_{\tau \sim q\left(\tau\right)}\sum_{\psi}p\left(\psi | \tau\right)U_{\psi}\left(\tau\right) 
% \end{equation*}
% Without any relabeling, the meta-RL objective becomes:
% \begin{equation*}
%     \mathbb{E}_{p\left(\psi, \tau\right)}\left[U_{\psi}\left(\tau\right)\right] = \int_{\tau \sim q\left(\tau\right)}U_{\psi_{\tau}}\left(\tau\right)
% \end{equation*}
% where $p\left(\psi_{\tau} | \tau\right)$ is 1 for the original task $\psi$ that trajectory $\tau$ was collected under. It is clear that to maximize the objective, we should assign trajectory $\tau$ to task $\psi_{\text{max}}^{\tau}$ under which $\tau$ achieves the maximum utility among all tasks. Given this relabeling scheme, the meta-RL objective becomes:
% \begin{equation*}
%     \mathbb{E}_{p\left(\psi, \tau\right)}\left[U_{\psi}\left(\tau\right)\right] = \int_{\tau \sim q\left(\tau\right)}U_{\psi_{\text{max}}^{\tau}}\left(\tau\right) \geq \int_{\tau \sim q\left(\tau\right)}U_{\psi_{\tau}}\left(\tau\right)
% \end{equation*}
% This is clearly the relabeling distribution that maximizes the meta-RL objective.
% \end{proof}
% Note that we can relabel using both normalized utility and unnormalized utility; we choose to use the normalized utility due to the possibility of different reward ranges across tasks, as well as differences in task difficulty. Also note that we can choose to view the relabeling process through the lens of a policy $\pi\left(\psi | \tau\right)$ that must choose which task to assign a trajectory to, and that the softmax task distribution $\pi\left(\psi | \tau\right)$ has positive entropy while the hard max task distribution has zero entropy, as all the probability mass is placed on a single task. (Maybe further explain connection to MaxEnt RL here) Our results when using max-relabeling can be seen in Figure~\ref{fig:hardmax_ablation}.

==> partition_algo.tex <==
\RestyleAlgo{ruled}
\begin{algorithm}[h!]
\SetNoFillComment
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{$\psi$: task to compute partition function for}
\Output{$\log Z\left(\psi\right)$: log of the partition function}
\BlankLine
Sample batch of trajectories $\left\{\tau^i\right\}_{i=1}^N \sim B_{\psi}$ \\
\For{each trajectory $\tau^i$}{
    Compute utility $U_{\psi}\left(\tau^i\right)$ using either Algorithm~\ref{algo:hfr_utility_return} or Algorithm~\ref{algo:hfr_utility_bellman}
}
$\log Z\left(\psi\right) = \log\left(\frac{1}{N}\sum_{i=1}^{N}e^{U_{\psi}\left(\tau^i\right)}\right)$
\caption{Computation of Partition Function}
\label{algo:partition}
\end{algorithm}

==> utility_returns_algo.tex <==
\RestyleAlgo{ruled}
\floatname{algorithm}{Procedure 1}
\begin{algorithm}[t]
\renewcommand{\thealgorithm}{}
\SetNoFillComment
\DontPrintSemicolon
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input{Trajectory to be relabeled ($\tau$) \newline
Task to compute utility of the trajectory for ($\psi$)}
\Output{Utility of the trajectory $\tau$ under task $\psi$, $U_{\psi}\left(\tau\right)$}
\BlankLine
\For{each $\left(s_t, a_t, r_t\right) \in \tau$}{
Replace $r_t$ with $r_{\psi}\left(s_t, a_t\right)$
}
Sample embedding using the encoder $z \sim q_{\phi}\left(z | \tau\right)$ 

Sample a batch of initial states $\left\{s_1^i\right\}_{i=1}^N \sim B_{\psi}$ 

Sample actions for these states using the post-adaptation policy $\pi_\theta(\cdot|s,z)$: $\left\{a_1 \sim \pi_{\theta}\left(a_1^i | s_1^i, z\right)\right\}_{i=1}^N$ 

Compute empirical estimation of the state-action value: $U_{\psi} = \frac{1}{N}\sum_{i=1}^N Q_{\theta}\left(s_1^i, a_1^i, z\right)$ \Comment*[r]{Eq.~\ref{eq:utility_postAdap}}

\caption{Computation of the utility function (Eq.~\ref{eq:utility_postAdap}), for PEARL-based meta-RL}
\label{algo:hfr_utility_return}
\end{algorithm}
\floatname{algorithm}{Algorithm}
